DynaVis: Dynamically Synthesized UI Widgets for Visualization Editing

Users often rely on GUIs to edit and interact with visualizations - a daunting task due to the large space of editing options. As a result, users are either overwhelmed by a complex UI or constrained by a custom UI with a tailored, fixed subset of options with limited editing flexibility. Natural Language Interfaces (NLIs) are emerging as a feasible alternative for users to specify edits. However, NLIs forgo the advantages of traditional GUI: the ability to explore and repeat edits and see instant visual feedback. We introduce DynaVis, which blends natural language and dynamically synthesized UI widgets. As the user describes an editing task in natural language, DynaVis performs the edit and synthesizes a persistent widget that the user can interact with to make further modifications. Study participants (n=24) preferred DynaVis over the NLI-only interface citing ease of further edits and editing confidence due to immediate visual feedback.

==> 05.1-task-table.tex <==
\begin{table}[t]
\centering
\begin{tabularx}{\textwidth}{|p{0.8in}|X|X|X|}
\hline
& \textbf{Task 1. Stock Trends} & \textbf{Task 2. Unemployment Data} & \textbf{Task 3. Weather Data} \\ \hline

\textbf{Sub-task 1} & Change the chart title to "Stock Trend" & Change the x-axis title to "Timeline" & Change the y-axis title to "Number of Records" \\ \hline

\textbf{Sub-task 2} & Try out different stroke width for the lines in the chart to find the best thickness that suits you. & Try out different legend position (external and internal) and choose the best position that suits you. & Rotate the x-axis labels by 45, 65, 90 degrees and choose the best angle that suits you. \\ \hline

\textbf{Sub-task 3} & Edit the chart to show the stock trends for AAPL and MSFT only. & Edit the chart to show the trend only for Construction and Agriculture sectors. & Change the color of each weather type to the following colors: Sun to Yellow, Snow to Gray, Rain to Blue, Fog to Green, Drizzle to Purple. \\ \hline

\textbf{Sub-task 4} & Change the y-axis max range to 250 to get a zoomed in view. \newline \newline \textit{Question}: By just viewing the chart, get the minimum and maximum stock price for both AAPL and MSFT & Edit the y-axis max date to 06/01/2004 (1 June 2004). \newline \newline \textit{Question}: By just viewing the chart, get the approximate month and year, where the difference in unemployment rate between the two sectors were maximum. & Edit the chart to only show Snow weather type for all the months.\newline \newline  \textit{Question}: By just viewing the chart, find the month with the lowest snow days.  \\ \hline

\textbf{Sub-task 5} & Now compare only between IBM and MSFT. \newline \newline \textit{Question}: By just viewing the chart, find the month and year, where the difference in stock price between the two companies were maximum. & Now compare only between Finance and Construction sector.\newline \newline  \textit{Question}: By just viewing the chart, get the approximate month and year, where the difference in unemployment rate between the two sectors were maximum. & Now edit the chart to only show Fog weather type for all the months.\newline \newline  \textit{Question}: By just viewing the chart, find the month with the highest fog days. \\ \hline

\textbf{Base \newline Visualization} & 
\begin{minipage}{\linewidth} \includegraphics[width=\linewidth]{res/task1.png} \end{minipage} & 
\begin{minipage}{\linewidth} \includegraphics[width=\linewidth]{res/task2.png} \end{minipage} & 
\begin{minipage}{\linewidth} \includegraphics[width=\linewidth]{res/task3.png} \end{minipage} \\ \hline

\end{tabularx}
\caption{List of tasks for the user study}
\label{tab:tasks}
\end{table}
